Constructing Intrinsic Delaunay Triangulations of Submanifolds

We describe an algorithm to construct an intrinsic Delaunay triangulation of a smooth closed submanifold of Euclidean space. Using results established in a companion paper on the stability of Delaunay triangulations on $\delta$-generic point sets, we establish sampling criteria which ensure that the intrinsic Delaunay complex coincides with the restricted Delaunay complex and also with the recently introduced tangential Delaunay complex. The algorithm generates a point set that meets the required criteria while the tangential complex is being constructed. In this way the computation of geodesic distances is avoided, the runtime is only linearly dependent on the ambient dimension, and the Delaunay complexes are guaranteed to be triangulations of the manifold.

==> abstract_con.tex <==
% -*- LaTeX -*-
% abstract_con.tex
% 20120504
% for Delaunay construction stability paper

\begin{abstract}
  We describe an algorithm to construct an intrinsic Delaunay
  triangulation of a smooth closed submanifold of Euclidean space.
  Using results established in a companion paper on the stability of
  Delaunay triangulations on $\delta$-generic point sets, we establish
  sampling criteria which ensure that the intrinsic Delaunay complex
  coincides with the restricted Delaunay complex and also with the
  recently introduced tangential Delaunay complex.  The algorithm
  generates a point set that meets the required criteria while the
  tangential complex is being constructed.  In this way the
  computation of geodesic distances is avoided, the runtime is only
  linearly dependent on the ambient dimension, and the Delaunay
  complexes are guaranteed to be triangulations of the manifold.
\end{abstract}

